Scratchpad Sharing in GPUs

GPGPU applications exploit on-chip scratchpad memory available in the Graphics Processing Units (GPUs) to improve performance. The amount of thread level parallelism present in the GPU is limited by the number of resident threads, which in turn depends on the availability of scratchpad memory in its streaming multiprocessor (SM). Since the scratchpad memory is allocated at thread block granularity, part of the memory may remain unutilized. In this paper, we propose architectural and compiler optimizations to improve the scratchpad utilization. Our approach, Scratchpad Sharing, addresses scratchpad under-utilization by launching additional thread blocks in each SM. These thread blocks use unutilized scratchpad and also share scratchpad with other resident blocks. To improve the performance of scratchpad sharing, we propose Owner Warp First (OWF) scheduling that schedules warps from the additional thread blocks effectively. The performance of this approach, however, is limited by the availability of the shared part of scratchpad. We propose compiler optimizations to improve the availability of shared scratchpad. We describe a scratchpad allocation scheme that helps in allocating scratchpad variables such that shared scratchpad is accessed for short duration. We introduce a new instruction, relssp, that when executed, releases the shared scratchpad. Finally, we describe an analysis for optimal placement of relssp instructions such that shared scratchpad is released as early as possible. We implemented the hardware changes using the GPGPU-Sim simulator and implemented the compiler optimizations in Ocelot framework. We evaluated the effectiveness of our approach on 19 kernels from 3 benchmarks suites: CUDA-SDK, GPGPU-Sim, and Rodinia. The kernels that underutilize scratchpad memory show an average improvement of 19% and maximum improvement of 92.17% compared to the baseline approach.

==> Makefile <==
TGT=CompOptJournal

BIBTEX=bibtex
LATEX=pslatex
DVIPS=dvips
PS2PDF=ps2pdf
# Ignore these for now!
#PS2PDF_OPTS=-dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true -dPDFSETTINGS=/prepress 
#LATEX_OPTS=-interaction=nonstopmode -halt-on-error
LATEX_OPTS=

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"


.PHONY: all clean

all: $(TGT).pdf

$(TGT).dvi : $(TGT).tex Sections/*.tex pstImages/*.tex CompOptJournal.bib ReleaseSSP.c
	$(LATEX) $(LATEX_OPTS) $(TGT).tex
	@if(grep "There were undefined references" $(TGT).log > /dev/null);\
	then \
		$(BIBTEX) $(TGT).aux; \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex; \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex; \
	fi
	@if(grep "Rerun" $(TGT).log > /dev/null);\
	then \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex;\
	fi

$(TGT).ps: $(TGT).dvi
	$(DVIPS) -j0 $<

$(TGT).pdf: $(TGT).ps
	$(PS2PDF) $<

clean:
	$(RM) $(TGT).aux $(TGT).log   \
		$(TGT).blg $(TGT).bbl \
		$(TGT).dvi $(TGT).out \
		$(TGT).pdf $(TGT).ps


==> Sections/00-todo.tex <==
\tbd{
\section*{TODO before final submission}
\begin{enumerate}
\item replace {\em access range} by {\em live range}
\item check space after \Release.
\item Spell check
\item remove this section
\item replace resource with scratchpad accordingly
\item Write hardware requirement section, and compute the number of extra bits require to model the latency of \Release\ instruction
\end{enumerate}
}


==> Sections/05-SystemImpl.tex <==
\newcommand{\SM}{\mbox{SM}}
\section{System Implementation} \label{sec:systemImpl}


\begin{figure}[t]
\centering
\includegraphics[scale=0.25]{Images/System.eps}
%\vskip 1mm
\caption{System Implementation}
\label{fig:system}
%\vskip -3mm
\end{figure}

Figure~\ref{fig:system} illustrates the overall implementation of our approach. We implemented the proposed compiler optimizations in the Ocelot PTX transformation framework. We integrated the new hardware \Release\ instruction in the GPGPU-Simulator that supports resource sharing approach.


Consider an application {\tt Input.cu}, which is written in CUDA as shown in the Figure, that needs to be analyzed for performance using GPU simulator. We compile the input program using {\tt nvcc} compiler that produces an executable file, {\tt a.out},  as indicated. The executable is converted into a PTX assembly using the {\tt cuobjdump } tool. The intermediate PTX is transformed to optimized PTX code using the Ocelot framework that has our optimizations. The transformed PTX (which contains the \Release\ instruction) is simulated using our modified resource sharing GPGPU-Sim simulator. To compare the performance our approach, we processed the original PTX using the Ocelot framework that does not contain optimization. Further we simulate this PTX using the existing the Resource sharing GPGPU-Sim simulator.

\ak{Are you not stating the obvious? Is there any other ``correct'' way to show the effectiveness of your optimizations? Why waste a figure and two paragraphs. I do not see why we should have this section at all!!}




==> pstImages/Unshared.tex <==
\newcommand{\Warp}[2]{%
\psset{unit=.25mm}
\begin{pspicture}(0,0)(40,20)
\psframe(0,0)(40,20)
\putnode{zarb1342}{origin}{20}{10}{\rnode{#1}{#2}}
\end{pspicture}%
}

\begin{figure}[t]
\centering
\renewcommand{\arraystretch}{0.99}
\begin{tabular}{c c}
\scalebox{.9}{
\psset{unit=1mm}
\psset{linewidth=.3mm}
\begin{pspicture}(1,3)(63,48)
  \psframe(1,2)(63,48)
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \putnode{t0}{origin}{32}{45}{Scratchpad Size per SM = 35KB}

  \psframe(5,9)(21,34)
  \putnode{o1}{origin}{13}{25}{\rnode{r0}{}}
  \putnode{o2}{o1}{0}{-3}{\rnode{r1}{10 Warps}}
  \putnode{t1}{o2}{0}{16}{\begin{tabular}{c}TB$_0$\\(10KB)\end{tabular}}
  \putnode{t2}{o2}{0}{-17}{\begin{tabular}{c}Unshared\end{tabular}}

  \psframe(24,9)(40,34)
  \putnode{o1}{origin}{32}{25}{\rnode{r0}{}}
  \putnode{o2}{o1}{0}{-3}{\rnode{r1}{10 Warps}}
  \putnode{t1}{o2}{0}{16}{\begin{tabular}{c}TB$_1$\\(10KB)\end{tabular}}
  \putnode{t2}{o2}{0}{-17}{\begin{tabular}{c}Unshared\end{tabular}}


  \psframe(43,9)(59,34)
  \putnode{o1}{origin}{51}{25}{\rnode{r0}{}}
  \putnode{o2}{o1}{0}{-3}{\rnode{r1}{10 Warps}}
  \putnode{t1}{o2}{0}{16}{\begin{tabular}{c}TB$_2$\\(10KB)\end{tabular}}
  \putnode{t2}{o2}{0}{-17}{\begin{tabular}{c}Unshared\end{tabular}}

\end{pspicture}}
& 
\scalebox{.9}{
\psset{unit=1mm}
\psset{linewidth=.3mm}
\begin{pspicture}(1,3)(82,48)
  \psframe(1,2)(82,48)
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \putnode{t0}{origin}{41}{45}{Scratchpad Size per SM = 35KB}

  \psframe(5,9)(21,34)
  \putnode{o1}{origin}{13}{25}{\rnode{r0}{}}
  \putnode{o2}{o1}{0}{-3}{\rnode{r1}{10 Warps}}
  \putnode{t1}{o2}{0}{16}{\begin{tabular}{c}TB$_0$\\(10KB)\end{tabular}}
  \putnode{t2}{o2}{0}{-17}{\begin{tabular}{c}Unshared\end{tabular}}
  

  \psframe(24,9)(40,34)
  \putnode{o1}{origin}{32}{25}{\rnode{r0}{}}
  \putnode{o2}{o1}{0}{-3}{\rnode{r1}{10 Warps}}
  \putnode{t1}{o2}{0}{16}{\begin{tabular}{c}TB$_1$\\(10KB)\end{tabular}}
  \putnode{t2}{o2}{0}{-17}{\begin{tabular}{c}Unshared\end{tabular}}
  

  \putnode{o21}{origin}{50}{25}{\rnode{r0}{}}
  \putnode{o22}{o21}{0}{-3}{\rnode{r1}{10 Warps}}
  \putnode{o23}{o22}{0}{-5}{}  
  \putnode{o29}{o23}{0}{-6}{}
  \putnode{t1}{o22}{0}{17}{\begin{tabular}{c}TB$_2$\\\ \end{tabular}}
  \putnode{t1a}{t1}{-8}{-1}{}
  \putnode{t2a}{o29}{-8}{-6}{}

  \putnode{o31}{origin}{72}{25}{\rnode{r0}{}}
  \putnode{o32}{o31}{0}{-3}{\rnode{r1}{10 Warps}}
  \putnode{o33}{o32}{0}{-5}{}  
  \putnode{o39}{o33}{0}{-6}{}
  \putnode{t1}{o32}{0}{17}{\begin{tabular}{c}TB$_3$\\\ \end{tabular}}
  \putnode{t1b}{t1}{7}{-1}{}
  \putnode{t2b}{o39}{7}{-6}{}

  \ncline{|-|}{t2a}{t2b} \lput*{:U}{Shared}
  \ncline{|-|}{t1a}{t1b} \lput*{:U}{(15KB)}
  \psframe(64,9)(79,34)
  \psframe(42,9)(58,34)

  \putnode{s29}{o29}{1}{10}{}
  \putnode{s39}{s29}{19}{0}{}
  \ncline[nodesepA=17pt,nodesepB=15pt,doubleline=true]{<->}{s29}{s39}
\end{pspicture}}
\\ (a)  & (b) \\ \\
\end{tabular}
\vskip -3mm
\caption{ Scratchpad Memory Allocation Schemes: (a) Default Approach (b)  Scratchpad Sharing\label{fig:resourcealloc} }
\vskip -4mm
\end{figure}


